Les Houches 2019 Physics at TeV Colliders: New Physics Working Group Report

This report presents the activities of the `New Physics' working group for the `Physics at TeV Colliders' workshop (Les Houches, France, 10--28 June, 2019). These activities include studies of direct searches for new physics, approaches to exploit published data to constrain new physics, as well as the development of tools to further facilitate these investigations. Benefits of machine learning for both the search for new physics and the interpretation of these searches are also presented.

==> 2hdm/2hdma.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  J.~M.~Butterworth$^{UCL}$,
  M.Habedank$^{HU}$,
  P.~Pani$^{DESY}$
\end{flushleft}

\begin{itemize}
\item[$^{UCL}$] Department of Physics and Astronomy, UCL, London, WC1E 6BT, UK
\item[$^{HU}$] Department of Physics, HU Berlin, Germany
\item[$^{DESY}$] DESY Zeuthen, Berlin, Germany
\end{itemize}




==> 4top/4top.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  D.~Kar$^{Wits}$,
  L.~Corpe$^{UCL}$
\end{flushleft}

\begin{itemize}
\item[$^{Wits}$] School of Physics, University of Witwatersrand, Johannesburg, South Africa
\item[$^{UCL}$] Department of Physics, University College London, London, UK
\end{itemize}




==> 4top/4top.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}


==> HiggsZa/HiggsZa.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
 A. Bharucha$^{CPT}$, 
 J. M. Butterworth$^{UCL}$, 
 N. Desai$^{TIFR}$, 
 S. Gascon-Shotkin$^{IPNL}$, 
 S. Jain$^{UMN}$, 
 A. Lesauvage$^{IPNL}$, 
 G. Moreau$^{IJCLab}$, 
 S. Mutzel$^{CPT}$, 
 J. M. No$^{UAMCSIC}$, 
 J. Quevillon$^{IN2P3Gr}$, 
 C. Smith$^{IN2P3Gr}$, 
 K. Tobioka$^{FLD}$, 
 N. Vignaroli$^{FisPisa}$, 
 S. L. Williamson$^{LPTHE,ITP}$, 
 J. Zurita$^{IKP,TTP}$
\end{flushleft}

\begin{itemize}
\item[$^{CPT}$] CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{UCL}$] Department of Physics and Astronomy, UCL, London, UK
\item[$^{TIFR}$] Department of Theoretical Physics, Tata Institute of Fundamental Research, Mumbai, India
\item[$^{IPNL}$] Univ. Lyon, Universit\'e Claude Bernard Lyon 1, CNRS/IN2P3, UMR5822 IPNL F-69622 Villeurbanne, France
\item[$^{UMN}$] University of Minnesota, Minneapolis, MN 55455, United States 
\item[$^{IJCLab}$] Laboratoire de Physique des 2 Infinis Ir\`ene Joliot-Curie d'Orsay (IJCLab), B\^at. 100, CNRS / PARIS-SACLAY, F-91898 ORSAY Cedex, France
\item[$^{UAMCSIC}$] Departamento de Fisica Teorica and Instituto de Fisica Teorica, IFT-UAM/CSIC, Cantoblanco, 28049, Madrid, Spain
%\item[$^{8}$] Instituto de Fisica Teorica, IFT-UAM/CSIC,Cantoblanco, 28049, Madrid, Spain
\item[$^{IN2P3Gr}$] Laboratoire de Physique Subatomique et de Cosmologie, Université Grenoble-Alpes, CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{FLD}$] Department of Physics, Florida State University, Tallahassee, FL 32306, USA
\item[$^{FisPisa}$] Dipartimento di Fisica "E. Fermi", Università di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE),UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{ITP}$] Institute for Theoretical Physics (ITP), Karlsruhe Institute of Technology, 76128 Karlsruhe, Germany
\item[$^{IKP}$] Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology, 
Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, 
Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> adl/LH19ADLoverlap.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  H.~B.~Prosper$^{FSU}$,
  S.~Sekmen$^{KNU}$,
  W.~Waltenberger$^{OAW}$
\end{flushleft}

\begin{itemize}
\item[$^{FSU}$] Department of Physics, Florida State University, Tallahassee, Florida 32306, USA
\item[$^{KNU}$] Department of Physics, Kyungpook National University, Daegu, South Korea
\item[$^{OAW}$] Institut f\"ur Hochenergiephysik, \"Osterreichische Akademie der Wissenschaften, Nikolsdorfer Gasse 18, 1050 Wien, Austria
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> adl/LH19ADLoverlap.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}


==> anacor/BSM_AnalysisCorrelations.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
A.~Buckley$^{1}$,
B.~Fuks$^{2,3}$,
H.~Reyes-Gonz\'alez$^{4}$,
W.~Waltenberger$^{5}$,
S.~L.~Williamson$^{2,6}$.
\end{flushleft}

\begin{itemize}
\item[$^{1}$]{School of Physics \& Astronomy, University of Glasgow, Glasgow, Scotland, UK}
\item[$^{2}$] {Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE),UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France}
\item[$^{3}$]{Institut Universitaire de France, 103 Boulevard Saint-Michel,  75005 Paris, France}
\item[$^{4}$]{Laboratoire de Physique Subatomique et de Cosmologie, Université Grenoble-Alpes, CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France}
\item[$^{5}$]{Institut f\"ur Hochenergiephysik,  \"Osterreichische Akademie der  Wissenschaften, Nikolsdorfer Gasse 18, 1050 Wien, Austria}
\item[$^{6}$] {Institute for Theoretical Physics, Karlsruhe Institute of Technology,
76128 Karlsruhe, Germany}
\end{itemize}



==> anacor/BSM_AnalysisCorrelations.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{graphicx}
\usepackage{color}
\usepackage{fullpage}
\usepackage{mathrsfs}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{verbatim}
\usepackage{hyperref}
\usepackage{url}
%\usepackage{authblk}
\usepackage{latexsym}
\usepackage{subfigure}
%\usepackage{subcaption}
\usepackage{cleveref}
\usepackage{ulem}
%\usepackage{breakcites}
%\usepackage{microtype}
%\definecolor{darkmagenta}{rgb}{0.55, 0.0, 0.55}
%\newcommand{\benj}[1]{{\color{darkmagenta}#1}}



==> authors-files/2hdma.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  J.~M.~Butterworth$^{UCL}$,
  M.~Habedank$^{HU}$,
  P.~Pani$^{DESY}$
\end{flushleft}

\begin{itemize}
\item[$^{UCL}$] Department of Physics and Astronomy, UCL, London, WC1E 6BT, UK
\item[$^{HU}$] Department of Physics, HU Berlin, Germany
\item[$^{DESY}$] DESY Zeuthen, Berlin, Germany
\end{itemize}




==> authors-files/4top.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  D.~Kar$^{Wits}$,
  L.~Corpe$^{UCL}$
\end{flushleft}

\begin{itemize}
\item[$^{Wits}$] School of Physics, University of Witwatersrand, Johannesburg, South Africa
\item[$^{UCL}$] Department of Physics, University College London, London, UK
\end{itemize}




==> authors-files/BSM_AnalysisCorrelations.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
A.~Buckley$^{1}$,
B.~Fuks$^{2}$,
B.~Fuks$^{3}$,
H.~ReyesGonzalez$^{4}$,
W.~Waltenberger$^{5}$,
S.~L.~Williamson$^{2}$,
S.~L.~Williamson$^{6}$.
\end{flushleft}

\begin{itemize}
\item[$^{1}$]{School of Physics \& Astronomy, University of Glasgow, Glasgow, Scotland, UK}
\item[$^{2}$] {Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE),UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France}
\item[$^{3}$]{Institut Universitaire de France, 103 Boulevard Saint-Michel,  75005 Paris, France}
\item[$^{4}$]{Laboratoire de Physique Subatomique et de Cosmologie, Université Grenoble-Alpes, CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France}
\item[$^{5}$]{Institut f\"ur Hochenergiephysik,  \"Osterreichische Akademie der  Wissenschaften, Nikolsdorfer Gasse 18, 1050 Wien, Austria}
\item[$^{6}$] {Institute for Theoretical Physics, Karlsruhe Institute of Technology,
76128 Karlsruhe, Germany}
\end{itemize}



==> authors-files/FILC.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  G.~Belanger$^{LAPTh}$,
  A.~Bharucha$^{CPT}$,
  N.~Desai$^{TIFR}$, 
  B.~Fuks$^{LPTHE}$,
  B.~Fuks$^{IUF}$,
  A.~Goudelis$^{LPC}$,
  J.~Heisig$^{CP3}$,
  A.~Lessa$^{ABC}$,
  A.~Mjallal$^{LAPTh}$,
  S.~Sekmen$^{Kyungpook}$,
  D.~Sengupta$^{UCSD}$,
  J.~Zurita$^{IKP}$,
  J.~Zurita$^{TTP}$  
\end{flushleft}

\begin{itemize}
\item[$^{LAPTh}$] LAPTh, Univ.\ Grenoble Alpes, USMB, CNRS, 9 Chemin de Bellevue, F74940 Annecy, France
\item[$^{CPT}$] CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{TIFR}$] Department of Theoretical Physics, Tata Institute of Fundamental Research, Homi Bhabha Road, Mumbai 400005, India
\item[$^{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{LPC}$] Laboratoire de Physique de Clermont (UMR 6533), CNRS/IN2P3, Univ.\ Clermont Auvergne, 4 Av.\ Blaise Pascal, F-63178 Aubi\`ere Cedex, France
\item[$^{CP3}$] Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{ABC}$] Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil
\item[$^{Kyungpook}$] Department of Physics, Kyungpook National University, Daegu, South Korea
\item[$^{UCSD}$] Department of Physics and Astronomy, University of California, San Diego, 9500 Gilman Drive, La Jolla, U.S.A
\item[$^{IKP}$] Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology, Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/GWC.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  J.~M.~Butterworth$^{1}$,
  K.~Lane$^{2}$,
  D.~Sperka$^{2}$
\end{flushleft}

\begin{itemize}
\item[$^{1}$] Department of Physics \& Astronomy, University College London, London, UK
\item[$^{2}$] Department of Physics, Boston University, Boston, MA 02215, USA
\end{itemize}


\title{Confronting the Higgs Bosons in Gildener-Weinberg Models with LHC
  Measurements}
\author{Jonathan~M.~Butterworth$^{1}$, Kenneth Lane$^{2}$}
\institute{
$^{1}$Department of Physics \& Astronomy, UCL, London, UK\\
$^{2}$Department of Physics, Boston University, Boston, MA 02215, USA
}



==> authors-files/HiggsZa.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
 A.~Bharucha$^{CPT}$, 
 J.~M.~Butterworth$^{UCL}$, 
 N.~Desai$^{TIFR}$, 
 S.~GasconShotkin$^{IPNL}$, 
 S.~Jain$^{UMN}$, 
 A.~Lesauvage$^{IPNL}$, 
 G.~Moreau$^{IJCLab}$, 
 S.~Mutzel$^{CPT}$, 
 J.~M.~No$^{UAMCSIC}$, 
 J.~Quevillon$^{IN2P3Gr}$, 
 C.~Smith$^{IN2P3Gr}$, 
 K.~Tobioka$^{FLD}$, 
 N.~Vignaroli$^{FisPisa}$, 
 S.~L.~Williamson$^{LPTHE}$, 
 S.~L.~Williamson$^{ITP}$, 
 J.~Zurita$^{IKP}$,
 J.~Zurita$^{TTP}$
\end{flushleft}

\begin{itemize}
\item[$^{CPT}$] CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{UCL}$] Department of Physics and Astronomy, UCL, London, UK
\item[$^{TIFR}$] Department of Theoretical Physics, Tata Institute of Fundamental Research, Mumbai, India
\item[$^{IPNL}$] Univ. Lyon, Universit\'e Claude Bernard Lyon 1, CNRS/IN2P3, UMR5822 IPNL F-69622 Villeurbanne, France
\item[$^{UMN}$] University of Minnesota, Minneapolis, MN 55455, United States 
\item[$^{IJCLab}$] Laboratoire de Physique des 2 Infinis Ir\`ene Joliot-Curie d'Orsay (IJCLab), B\^at. 100, CNRS / PARIS-SACLAY, F-91898 ORSAY Cedex, France
\item[$^{UAMCSIC}$] Departamento de Fisica Teorica and Instituto de Fisica Teorica, IFT-UAM/CSIC, Cantoblanco, 28049, Madrid, Spain
%\item[$^{8}$] Instituto de Fisica Teorica, IFT-UAM/CSIC,Cantoblanco, 28049, Madrid, Spain
\item[$^{IN2P3Gr}$] Laboratoire de Physique Subatomique et de Cosmologie, Université Grenoble-Alpes, CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{FLD}$] Department of Physics, Florida State University, Tallahassee, FL 32306, USA
\item[$^{FisPisa}$] Dipartimento di Fisica "E. Fermi", Università di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE),UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{ITP}$] Institute for Theoretical Physics (ITP), Karlsruhe Institute of Technology, 76128 Karlsruhe, Germany
\item[$^{IKP}$] Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology, 
Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, 
Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/LH19ADLoverlap.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  H.~B.~Prosper$^{FSU}$,
  S.~Sekmen$^{KNU}$,
  W.~Waltenberger$^{OAW}$
\end{flushleft}

\begin{itemize}
\item[$^{FSU}$] Department of Physics, Florida State University, Tallahassee, Florida 32306, USA
\item[$^{KNU}$] Department of Physics, Kyungpook National University, Daegu, South Korea
\item[$^{OAW}$] Institut f\"ur Hochenergiephysik, \"Osterreichische Akademie der Wissenschaften, Nikolsdorfer Gasse 18, 1050 Wien, Austria
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/LLP_DM.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\title{A common solution to $R_D$ anomalies and Dark Matter}
\begin{flushleft}
B.~Fuks$^{LPTHE}$, 
B.~Fuks$^{IUF}$, 
J.~Heisig$^{CP3}$, 
A.~Lessa$^{UFABC}$, 
J.~M.~No$^{UAMCSIC}$,
S.~Sekmen$^{KNU}$,
D.~Sengupta$^{UCSD}$,
J.~Zurita$^{IKP}$.,
J.~Zurita$^{IKP}$. 
\end{flushleft}

\begin{itemize}
\item[ $^{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^\text{IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{CP3}$] Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{UFABC}$] Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil,
\item[$^{UAMCSIC}$] Departamento de Fisica Teorica and Instituto de Fisica Teorica, IFT-UAM/CSIC, Cantoblanco, 28049, Madrid, Spain,
\item[$^{KNU}$] Kyungpook National University, Physics Dept., Daegu, South Korea.
\item[$^{UCSD}$] Department of Physics and Astronomy, 9500 Gilman Drive, University of California, San Diego.
\item[$^{IKP}$] Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany,
\item[$^{TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology,  Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/PhenoAI.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  S.~Caron$^{IMAPP}$, 
  S.~Caron$^{Nikhef}$, 
  A.~Coccaro$^{INFN}$, 
  S.~Ganguly$^{WIS}$,
  S.~Kraml$^{LPSC}$, 
  A.~Lessa$^{UFABC}$, 
  S.~Otten$^{IMAPP}$, 
  S.~Otten$^{GRAPPA}$, 
  H.~ReyesGonzalez$^{LPSC}$, 
  R.~Ruiz$^{CP3}$, 
  R.~Ruiz~de~Austri$^{IFIC}$,
  B.~Stienen$^{IMAPP}$,
  B.~Stienen$^{Nikhef}$,
  R.~Torre$^{INFN}$
\end{flushleft}

\begin{itemize}
\item[$^{IMAPP}$]IMAPP, Radboud University, Nijmegen, the Netherlands
\item[$^{INFN}$]INFN, Sezione di Genova, Via Dodecaneso 33, I-16146 Genova, Italy
\item[$^{Nikhef}$]Nikhef, Amsterdam, the Netherlands
\item[$^{UFABC}$] Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil
\item[$^{CP3}$]Centre for Cosmology, Particle Physics and Phenomenology {\rm (CP3)}, Universit\'e Catholique de Louvain, Chemin du Cyclotron, Louvain la Neuve, B-1348, Belgium
\item[$^{LPSC}$]Laboratoire de Physique Subatomique et de Cosmologie, Universit\'{e} Grenoble-Alpes, \\ CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{IFIC}$]Instituto de F\'isica Corpuscular, IFIC-UV/CSIC, Valencia, Spain.
\item[$^{GRAPPA}$]GRAPPA, University of Amsterdam, the Netherlands
\item[$^{WIS}$] Weizmann Institute of Science, Israel
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/RDM.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\title{A common solution to $R_D$ anomalies and Dark Matter}
\begin{flushleft}
G.~Belanger$^{LAPTh}$, 
J.~Bernigaud$^{IKP}$, 
J.~Bernigaud$^{TTP}$, 
A.~Bharucha$^{CPT}$, 
B.~Fuks$^{LPTHE}$, 
B.~Fuks$^{IUF}$, 
J.~Heisig$^{CP3}$, 
A.~Jueid$^{LAPTh}$, 
A.~Goudelis$^{LPC}$, 
A.~Lessa$^{UFABC}$, 
D.~Marzocca$^{INFNTrieste}$,
K.~A.~Mohan$^{MSU}$,
M.~Nardecchia$^{Sapienza}$, 
G.~Polesello$^{INFNPavia}$, 
P.~Pani$^{DesyZ}$, 
A.~Pukhov$^{MGU}$, 
D.~Sengupta$^{UCSD}$,
J.~Zurita$^{IKP}$, 
J.~Zurita$^{TTP}$. 
\end{flushleft}

\begin{itemize}
\item[$^{LAPTh}$] LAPTh, Univ. Grenoble Alpes, USMB, CNRS, 9 Chemin de Bellevue, F-74940 Annecy, France
\item[$^{IKP}$] Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology,  Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\item[$^{CPT}$] CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{CP3}$] Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{Konkuk}$] School of Physics, Konkuk University, 05029, Seoul, Republic of Korea
\item[$^{LPC}$] Laboratoire de Physique de Clermont (UMR 6533), CNRS/IN2P3, Univ.\ Clermont Auvergne, 4 Av.\ Blaise Pascal, F-63178 Aubi\`ere Cedex, France
\item[$^{UFABC}$] Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil
\item[$^{INFNTrieste}$] INFN Sezione di Trieste, via Bonomea 265, 34136 Trieste, Italy 
\item[$^{MSU}$]  Department of Physics and Astronomy, 567 Wilson Road,  East Lansing, Michigan-48824, USA
\item[$^{Sapienza}$] Sapienza - Universita di Roma, Piazzale Aldo Moro 2, 00185, Roma, Italy
\item[$^{INFNPavia}$] INFN, Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy
\item[$^{DesyZ}$] Deutsches Elektronen Synchrotron, DESY, 15738 Zeuthen, Germany
\item[$^{MGU}$] Skobeltsyn Institute of Nuclear Physics, Moscow State University, Moscow 119992, Russia
\item[$^{UCSD}$] Department of Physics and Astronomy, 9500 Gilman Drive, University of California, San Diego
\end{itemize}


==> authors-files/SearchMeasurementComplementarity.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  T.~BergerHrynova$^{LAPP}$,
  A.~Buckley$^{UGlasgow}$,
  J.~M.~Butterworth$^{UCL}$,
  L.~Corpe$^{UCL}$,
  D.~Yallup$^{UCL}$,
  M.~van~Beekveld$^{UnivNijmegen}$,
  B.~Fuks$^{LPTHE}$,
  B.~Fuks$^{IUF}$,
  T.~Gonzalo$^{Monash}$,
  A.~Kvellestad$^{ICL}$,
  A.~Kvellestad$^{UnivOslo}$
\end{flushleft}

\begin{itemize}
\item[$^{LAPP}$] Univ.  Grenoble Alpes, Univ.  Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France
\item[$^{UGlasgow}$] School of Physics \& Astronomy, University of Glasgow, Scotland, UK
\item[$^{UCL}$] Department of Physics and Astronomy, University College London, UK
\item[$^{UnivNijmegen}$] Theoretical High Energy Physics, Radboud University Nijmegen, The Netherlands
\item[$^{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{Monash}$] School of Physics and Astronomy, Monash University, Melbourne, VIC 3800, Australia
\item[$^{ICL}$] Department of Physics, Imperial College London, UK
\item[$^{UnivOslo}$] Department of Physics, University of Oslo, Norway
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }


==> authors-files/VBF.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  S.~Fichet$^{IIP}$,
  S.~GasconShotkin$^{IPNL}$,
  A.~Lesauvage$^{IPNL}$, 
  G.~Moreau$^{IJCLab}$
\end{flushleft}

\begin{itemize}
\item[$^{IIP}$] International Institute of Physics, UFRN, Av. Odilon Gomes de Lima 1722 - Capim~Macio - 59078-400 - Natal-RN, Brazil
\item[$^{IPNL}$] Univ. Lyon, Universit\'e Claude Bernard Lyon 1, CNRS/IN2P3, UMR5822 IPNL F-69622 Villeurbanne, France
\item[$^{IJCLab}$] Laboratoire de Physique des 2 Infinis Ir\`ene Joliot-Curie d'Orsay (IJCLab), B\^at. 100, CNRS / PARIS-SACLAY, F-91898 ORSAY Cedex, France
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }

 


==> authors-files/all_authors.tex <==
\begin{flushleft}
G. Alguero$^{1}$, 
J. Y. Araz$^{2}$, 
J. Y. Araz$^{3}$, 
S. Banerjee$^{4}$, 
G. Belanger$^{5}$, 
G. Belanger$^{6}$, 
T. BergerHrynova$^{7}$, 
T. BergerHrynova$^{8}$, 
J. Bernigaud$^{9}$, 
J. Bernigaud$^{10}$, 
J. Bernigaud$^{11}$, 
J. Bernigaud$^{12}$, 
A. Bharucha$^{13}$, 
A. Bharucha$^{14}$, 
A. Bharucha$^{15}$, 
A. Bharucha$^{16}$, 
A. Buckley$^{17}$, 
A. Buckley$^{18}$, 
A. Buckley$^{19}$, 
A. Buckley$^{20}$, 
D. Buttazzo$^{21}$, 
D. Buttazzo$^{22}$, 
D. Buttazzo$^{23}$, 
J. M. Butterworth$^{24}$, 
J. M. Butterworth$^{25}$, 
J. M. Butterworth$^{26}$, 
J. M. Butterworth$^{27}$, 
J. M. Butterworth$^{28}$, 
S. Caron$^{29}$, 
S. Caron$^{30}$, 
A. Coccaro$^{31}$, 
L. Corpe$^{32}$, 
L. Corpe$^{33}$, 
L. Corpe$^{34}$, 
N. Desai$^{35}$, 
N. Desai$^{36}$, 
N. Desai$^{37}$, 
J. Dutta$^{38}$, 
J. Dutta$^{39}$, 
J. Dutta$^{40}$, 
J. Dutta$^{41}$, 
S. Fichet$^{42}$, 
B. Fuks$^{43}$, 
B. Fuks$^{44}$, 
B. Fuks$^{45}$, 
B. Fuks$^{46}$, 
B. Fuks$^{47}$, 
B. Fuks$^{48}$, 
B. Fuks$^{49}$, 
B. Fuks$^{50}$, 
B. Fuks$^{51}$, 
B. Fuks$^{52}$, 
B. Fuks$^{53}$, 
B. Fuks$^{54}$, 
B. Fuks$^{55}$, 
B. Fuks$^{56}$, 
S. Ganguly$^{57}$, 
S. GasconShotkin$^{58}$, 
S. GasconShotkin$^{59}$, 
A. Gilbert$^{60}$, 
T. Gonzalo$^{61}$, 
T. Gonzalo$^{62}$, 
A. Goudelis$^{63}$, 
A. Goudelis$^{64}$, 
P. Gras$^{65}$, 
R. S. Gupta$^{66}$, 
M. Habedank$^{67}$, 
J. Heisig$^{68}$, 
J. Heisig$^{69}$, 
J. Heisig$^{70}$, 
S. Jain$^{71}$, 
S. Jain$^{72}$, 
A. Jueid$^{73}$, 
D. Kar$^{74}$, 
S. Kraml$^{75}$, 
S. Kraml$^{76}$, 
A. Kvellestad$^{77}$, 
A. Kvellestad$^{78}$, 
A. Kvellestad$^{79}$, 
A. Kvellestad$^{80}$, 
K. Lane$^{81}$, 
J. Langford$^{82}$, 
A. Lesauvage$^{83}$, 
A. Lesauvage$^{84}$, 
A. Lessa$^{85}$, 
A. Lessa$^{86}$, 
A. Lessa$^{87}$, 
A. Lessa$^{88}$, 
D. Marzocca$^{89}$, 
D. Marzocca$^{90}$, 
D. Marzocca$^{91}$, 
D. Marzocca$^{92}$, 
A. Mjallal$^{93}$, 
K. A. Mohan$^{94}$, 
G. Moreau$^{95}$, 
G. Moreau$^{96}$, 
S. Mutzel$^{97}$, 
M. Nardecchia$^{98}$, 
M. Nardecchia$^{99}$, 
J. M. No$^{100}$, 
J. M. No$^{101}$, 
S. Otten$^{102}$, 
S. Otten$^{103}$, 
P. Pani$^{104}$, 
P. Pani$^{105}$, 
P. Pani$^{106}$, 
P. Pani$^{107}$, 
G. Polesello$^{108}$, 
G. Polesello$^{109}$, 
G. Polesello$^{110}$, 
H. B. Prosper$^{111}$, 
A. Pukhov$^{112}$, 
J. Quevillon$^{113}$, 
A. Raklev$^{114}$, 
H. ReyesGonzalez$^{115}$, 
H. ReyesGonzalez$^{116}$, 
R. Ruiz$^{117}$, 
R. Ruiz de Austri$^{118}$, 
R. Ruiz de Austri$^{119}$, 
S. Sekmen$^{120}$, 
S. Sekmen$^{121}$, 
S. Sekmen$^{122}$, 
S. Sekmen$^{123}$, 
D. Sengupta$^{124}$, 
D. Sengupta$^{125}$, 
D. Sengupta$^{126}$, 
C. Smith$^{127}$, 
M. Son$^{128}$, 
M. Son$^{129}$, 
D. Sperka$^{130}$, 
B. Stienen$^{131}$, 
B. Stienen$^{132}$, 
K. Tobioka$^{133}$, 
R. Torre$^{134}$, 
E. Venturini$^{135}$, 
E. Venturini$^{136}$, 
N. Vignaroli$^{137}$, 
N. Vignaroli$^{138}$, 
W. Waltenberger$^{139}$, 
W. Waltenberger$^{140}$, 
W. Waltenberger$^{141}$, 
N. Wardle$^{142}$, 
G. Watt$^{143}$, 
S. L. Williamson$^{144}$, 
S. L. Williamson$^{145}$, 
S. L. Williamson$^{146}$, 
S. L. Williamson$^{147}$, 
D. Yallup$^{148}$, 
D. Yallup$^{149}$, 
J. Zurita$^{150}$, 
J. Zurita$^{151}$, 
J. Zurita$^{152}$, 
J. Zurita$^{153}$, 
J. Zurita$^{154}$, 
J. Zurita$^{155}$, 
J. Zurita$^{156}$, 
J. Zurita$^{157}$, 
M. van Beekveld$^{158}$, 
\end{flushleft}

\begin{itemize}
\item[$^{116}$] Laboratoire de Physique Subatomique et de Cosmologie, Universit\'{e} Grenoble-Alpes, \\ CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{2}$]   Concordia University 7141 Sherbrooke St. West, Montr\'eal, QC, Canada H4B 1R6
\item[$^{3}$]  Department of Physics, Concordia University, Montr\'eal, Canada
\item[$^{143}$]  Institute for Particle Physics Phenomenology, Department of Physics, Durham University, Durham DH1 3LE, United Kingdom
\item[$^{93}$]  LAPTh, Univ. Grenoble Alpes, USMB, CNRS, 9 Chemin de Bellevue, F-74940 Annecy, France
\item[$^{93}$]  LAPTh, Univ. Grenoble Alpes, USMB, CNRS, 9 Chemin de Bellevue, F-74940 Annecy, France
\item[$^{8}$]  Univ.  Grenoble Alpes, Univ.  Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France
\item[$^{8}$]  Univ.  Grenoble Alpes, Univ.  Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France
\item[$^{156}$]  Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{157}$]  Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology,  Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\item[$^{156}$]  Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{157}$]  Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology,  Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\item[$^{97}$]  CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{97}$]  CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{97}$]  CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{97}$]  CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{26}$]  Department of Physics \& Astronomy, University College London, London, UK
\item[$^{18}$]  School of Physics and Astronomy, Glasgow University, Glasgow, UK
\item[$^{19}$]  School of Physics \& Astronomy, University of Glasgow, Scotland, UK
\item[$^{20}$]  School of Physics \& Astronomy, University of Glasgow, Scotland, UK
\item[$^{23}$]  INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{23}$]  INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{23}$]  INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{149}$]  Department of Physics and Astronomy, University College London, UK
\item[$^{149}$]  Department of Physics and Astronomy, University College London, UK
\item[$^{26}$]  Department of Physics \& Astronomy, University College London, London, UK
\item[$^{149}$]  Department of Physics and Astronomy, University College London, UK
\item[$^{149}$]  Department of Physics and Astronomy, University College London, UK
\item[$^{131}$] IMAPP, Radboud University, Nijmegen, the Netherlands
\item[$^{132}$] Nikhef, Amsterdam, the Netherlands
\item[$^{134}$] INFN, Sezione di Genova, Via Dodecaneso 33, I-16146 Genova, Italy
\item[$^{149}$]  Department of Physics and Astronomy, University College London, UK
\item[$^{149}$]  Department of Physics and Astronomy, University College London, UK
\item[$^{149}$]  Department of Physics and Astronomy, University College London, UK
\item[$^{37}$]  Department of Theoretical Physics, Tata Institute of Fundamental Research, Mumbai, India
\item[$^{37}$]  Department of Theoretical Physics, Tata Institute of Fundamental Research, Mumbai, India
\item[$^{37}$]  Department of Theoretical Physics, Tata Institute of Fundamental Research, Mumbai, India
\item[$^{40}$]  Regional Centre for Accelerator-based Particle Physics, Harish-Chandra Research Institute, HBNI, Chhatnag Road, Jhunsi, Allahabad-211019, India,
\item[$^{41}$]  II. Institut für Theoretische Physik, Universität Hamburg, Luruper Chaussee 149, 22761 Hamburg, Germany,
\item[$^{40}$]  Regional Centre for Accelerator-based Particle Physics, Harish-Chandra Research Institute, HBNI, Chhatnag Road, Jhunsi, Allahabad-211019, India,
\item[$^{41}$]  II. Institut für Theoretische Physik, Universität Hamburg, Luruper Chaussee 149, 22761 Hamburg, Germany,
\item[$^{42}$]  International Institute of Physics, UFRN, Av. Odilon Gomes de Lima 1722 - Capim~Macio - 59078-400 - Natal-RN, Brazil
\item[$^{144}$]  Department of Physics, Boston University, Boston, MA 02215, USA
\item[$^{44}$] {Institut Universitaire de France, 103 Boulevard Saint-Michel,  75005 Paris, France}
\item[$^{146}$]  Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{56}$]  Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{146}$]  Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{56}$]  Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{146}$]  Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{56}$]  Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{146}$]  Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{56}$]  Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{146}$]  Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{56}$]  Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{146}$]  Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{56}$]  Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{57}$]  Weizmann Institute of Science, Israel
\item[$^{84}$]  Univ. Lyon, Universit\'e Claude Bernard Lyon 1, CNRS/IN2P3, UMR5822 IPNL F-69622 Villeurbanne, France
\item[$^{84}$]  Univ. Lyon, Universit\'e Claude Bernard Lyon 1, CNRS/IN2P3, UMR5822 IPNL F-69622 Villeurbanne, France
\item[$^{60}$]  Northwestern University, Evanston, USA
\item[$^{62}$]  School of Physics and Astronomy, Monash University, Melbourne, VIC 3800, Australia
\item[$^{62}$]  School of Physics and Astronomy, Monash University, Melbourne, VIC 3800, Australia
\item[$^{64}$]  Laboratoire de Physique de Clermont (UMR 6533), CNRS/IN2P3, Univ.\ Clermont Auvergne, 4 Av.\ Blaise Pascal, F-63178 Aubi\`ere Cedex, France
\item[$^{64}$]  Laboratoire de Physique de Clermont (UMR 6533), CNRS/IN2P3, Univ.\ Clermont Auvergne, 4 Av.\ Blaise Pascal, F-63178 Aubi\`ere Cedex, France
\item[$^{65}$]  CEA Institut de Recherche sur les lois Fondamentales de l'Univers, Universit\'e Paris-Saclay, Gif-sur-Yvette, France
\item[$^{143}$]  Institute for Particle Physics Phenomenology, Department of Physics, Durham University, Durham DH1 3LE, United Kingdom
\item[$^{67}$]  Department of Physics, HU Berlin, Germany
\item[$^{117}$]  Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{117}$]  Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{117}$]  Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{71}$]  University of Minnesota, Minneapolis, MN 55455, United States 
\item[$^{72}$]  School of Physics \& Astronomy, University of Minnesota, Minneapolis MN 55455, United States of America
\item[$^{93}$]  LAPTh, Univ. Grenoble Alpes, USMB, CNRS, 9 Chemin de Bellevue, F-74940 Annecy, France
\item[$^{74}$]  School of Physics, University of Witwatersrand, Johannesburg, South Africa
\item[$^{116}$] Laboratoire de Physique Subatomique et de Cosmologie, Universit\'{e} Grenoble-Alpes, \\ CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{116}$] Laboratoire de Physique Subatomique et de Cosmologie, Universit\'{e} Grenoble-Alpes, \\ CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{79}$]  Department of Physics, Imperial College London, UK
\item[$^{114}$]  Department of Physics, University of Oslo, Norway
\item[$^{79}$]  Department of Physics, Imperial College London, UK
\item[$^{114}$]  Department of Physics, University of Oslo, Norway
\item[$^{144}$]  Department of Physics, Boston University, Boston, MA 02215, USA
\item[$^{142}$]  Imperial College, London, United Kingdom
\item[$^{84}$]  Univ. Lyon, Universit\'e Claude Bernard Lyon 1, CNRS/IN2P3, UMR5822 IPNL F-69622 Villeurbanne, France
\item[$^{84}$]  Univ. Lyon, Universit\'e Claude Bernard Lyon 1, CNRS/IN2P3, UMR5822 IPNL F-69622 Villeurbanne, France
\item[$^{85}$]  Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil
\item[$^{88}$]  Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil
\item[$^{88}$]  Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil
\item[$^{88}$]  Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil
\item[$^{92}$]  INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy
\item[$^{92}$]  INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy
\item[$^{92}$]  INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy
\item[$^{92}$]  INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy
\item[$^{93}$]  LAPTh, Univ. Grenoble Alpes, USMB, CNRS, 9 Chemin de Bellevue, F-74940 Annecy, France
\item[$^{94}$]   Department of Physics and Astronomy, 567 Wilson Road,  East Lansing, Michigan-48824, USA
\item[$^{96}$]  Laboratoire de Physique des 2 Infinis Ir\`ene Joliot-Curie d'Orsay (IJCLab), B\^at. 100, CNRS / PARIS-SACLAY, F-91898 ORSAY Cedex, France
\item[$^{96}$]  Laboratoire de Physique des 2 Infinis Ir\`ene Joliot-Curie d'Orsay (IJCLab), B\^at. 100, CNRS / PARIS-SACLAY, F-91898 ORSAY Cedex, France
\item[$^{97}$]  CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{99}$]  Sapienza - Universita di Roma, Piazzale Aldo Moro 2, 00185, Roma, Italy
\item[$^{99}$]  Sapienza - Universita di Roma, Piazzale Aldo Moro 2, 00185, Roma, Italy
\item[$^{101}$]  Departamento de Fisica Teorica and Instituto de Fisica Teorica, IFT-UAM/CSIC, Cantoblanco, 28049, Madrid, Spain,
\item[$^{101}$]  Departamento de Fisica Teorica and Instituto de Fisica Teorica, IFT-UAM/CSIC, Cantoblanco, 28049, Madrid, Spain,
\item[$^{131}$] IMAPP, Radboud University, Nijmegen, the Netherlands
\item[$^{103}$] GRAPPA, University of Amsterdam, the Netherlands
\item[$^{104}$]  DESY Zeuthen, Berlin, Germany
\item[$^{107}$]  Deutsches Elektronen Synchrotron, DESY, 15738 Zeuthen, Germany
\item[$^{106}$]  Deutsches Elektronen Synchrotron, DESY, 15738 Zeuthen, Germany
\item[$^{107}$]  Deutsches Elektronen Synchrotron, DESY, 15738 Zeuthen, Germany
\item[$^{110}$]  INFN, Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy
\item[$^{110}$]  INFN, Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy
\item[$^{110}$]  INFN, Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy
\item[$^{111}$]  Department of Physics, Florida State University, Tallahassee, Florida 32306, USA
\item[$^{112}$]  Skobeltsyn Institute of Nuclear Physics, Moscow State University, Moscow 119992, Russia
\item[$^{127}$]  Laboratoire de Physique Subatomique et de Cosmologie, UniversitÃ© Grenoble-Alpes, CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{114}$]  Department of Physics, University of Oslo, Norway
\item[$^{115}$] {Laboratoire de Physique Subatomique et de Cosmologie, UniversitÃ© Grenoble-Alpes, CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France}
\item[$^{116}$] Laboratoire de Physique Subatomique et de Cosmologie, Universit\'{e} Grenoble-Alpes, \\ CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{117}$]  Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{119}$]  Instituto de F\'isica Corpuscular, CSIC-Universitat de Val\`encia, Spain
\item[$^{119}$]  Instituto de F\'isica Corpuscular, CSIC-Universitat de Val\`encia, Spain
\item[$^{120}$]  Department of Physics, Kyungpook National University, Daegu, South Korea
\item[$^{123}$]  Department of Physics, Kyungpook National University, Daegu, South Korea
\item[$^{123}$]  Department of Physics, Kyungpook National University, Daegu, South Korea
\item[$^{123}$]  Department of Physics, Kyungpook National University, Daegu, South Korea
\item[$^{126}$]  Department of Physics and Astronomy, 9500 Gilman Drive, University of California, San Diego
\item[$^{126}$]  Department of Physics and Astronomy, 9500 Gilman Drive, University of California, San Diego
\item[$^{126}$]  Department of Physics and Astronomy, 9500 Gilman Drive, University of California, San Diego
\item[$^{127}$]  Laboratoire de Physique Subatomique et de Cosmologie, UniversitÃ© Grenoble-Alpes, CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{129}$]   Department of Physics, Korea Advanced Institute of Science and Technology, 291 Daehak-ro, Yuseong-gu, Daejeon 34141, Republic of Korea,
\item[$^{129}$]   Department of Physics, Korea Advanced Institute of Science and Technology, 291 Daehak-ro, Yuseong-gu, Daejeon 34141, Republic of Korea,
\item[$^{144}$]  Department of Physics, Boston University, Boston, MA 02215, USA
\item[$^{131}$] IMAPP, Radboud University, Nijmegen, the Netherlands
\item[$^{132}$] Nikhef, Amsterdam, the Netherlands
\item[$^{133}$]  Department of Physics, Florida State University, Tallahassee, FL 32306, USA
\item[$^{134}$] INFN, Sezione di Genova, Via Dodecaneso 33, I-16146 Genova, Italy
\item[$^{135}$]  Physik- Department, TUM, 85748 Garching, Germany
\item[$^{136}$]  Physik-Department, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany
\item[$^{138}$]  Dipartimento di Fisica "E. Fermi", UniversitÃ  di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{138}$]  Dipartimento di Fisica "E. Fermi", UniversitÃ  di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{139}$] {Institut f\"ur Hochenergiephysik,  \"Osterreichische Akademie der  Wissenschaften, Nikolsdorfer Gasse 18, 1050 Wien, Austria}
\item[$^{140}$]  Institut f\"ur Hochenergiephysik, \"Osterreichische Akademie der Wissenschaften, Nikolsdorfer Gasse 18, 1050 Wien, Austria
\item[$^{141}$]  Institut f\"ur Hochenergiephysik, \"Osterreichische Akademie der Wissenschaften, Nikolsdorfer Gasse 18, 1050 Wien, Austria
\item[$^{142}$]  Imperial College, London, United Kingdom
\item[$^{143}$]  Institute for Particle Physics Phenomenology, Department of Physics, Durham University, Durham DH1 3LE, United Kingdom
\item[$^{144}$]  Department of Physics, Boston University, Boston, MA 02215, USA
\item[$^{145}$]  {Institute for Theoretical Physics, Karlsruhe Institute of Technology,
\item[$^{146}$]  Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{147}$]  Institute for Theoretical Physics (ITP), Karlsruhe Institute of Technology, 76128 Karlsruhe, Germany
\item[$^{149}$]  Department of Physics and Astronomy, University College London, UK
\item[$^{149}$]  Department of Physics and Astronomy, University College London, UK
\item[$^{156}$]  Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{157}$]  Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology,  Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\item[$^{156}$]  Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{157}$]  Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology,  Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\item[$^{156}$]  Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{156}$]  Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{156}$]  Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{157}$]  Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology,  Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\item[$^{158}$]  Theoretical High Energy Physics, Radboud University Nijmegen, The Netherlands
\end{itemize}


==> authors-files/contur-update.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  A.~Buckley$^{Glasgow}$,
  J.~M.~Butterworth$^{UCL}$,
  L.~Corpe$^{UCL}$,
  G.~Watt$^{IPPP}$,
  D.~Yallup$^{UCL}$
\end{flushleft}

\begin{itemize}
\item[$^{Glasgow}$] School of Physics and Astronomy, Glasgow University, Glasgow, UK
\item[$^{UCL}$] Department of Physics and Astronomy, UCL, London, WC1E 6BT, UK 
\item[$^{IPPP}$] Institute for Particle Physics Phenomenology, Durham University, Durham, UK 
\end{itemize}




==> authors-files/darkmachines.authors.tex <==
\begin{flushleft}
 M.~van Beekveld$^{HEF,\,Nikhef}$,
 S.~Caron$^{HEF,\,Nikhef}$,
 A.~De Simone$^{SISSA,\,INFN}$,
 A.~Farbin$^{UnivArlington}$,
 L.~Hendriks$^{HEF}$,
 A.~Jueid$^{UnivKonkuk}$,
 A.~Leinweber$^{UnivAdelaide}$,
 J.~Mamuzic$^{IFIC}$,
 E.~Mer\'enyi$^{UnivRice}$,
 A.~Morandini$^{SISSA,\,INFN}$,
 C.~Nellist$^{HEF,\,Nikhef}$,
 S.~Otten$^{HEF,\,UnivAmsterdam}$,
 M.~Pierini$^{CERN}$,
 R.~Ruiz de Austri$^{IFIC}$,
  J.~Schouwenberg$^{HEF,\,Nikhef}$,
 S.~Sekmen$^{KNU}$,
 R.~Vilalta$^{UnivHouston}$,
 M.~White$^{UnivAdelaide}$
\end{flushleft}

\begin{itemize}
\item[$^{HEF}$] HEF, Radboud University, Nijmegen, the Netherlands\\
\item[$^{Nikhef}$] Nikhef, Amsterdam, the Netherlands\\
\item[$^{SISSA}$] SISSA, Trieste, Italy\\
\item[$^{INFN}$] INFN, Trieste, Italy\\
\item[$^{UnivArlington}$] University of Texas Arlington\\
\item[$^{UnivKonkuk}$] School of Physics, Konkuk University, Seoul, Republic of Korea\\
\item[$^{UnivAdelaide}$] University of Adelaide \\
\item[$^{IFIC}$] Instituto de F\'isica Corpuscular, IFIC-UV/CSIC, Valencia, Spain \\
\item[$^{UnivRice}$] Rice University\\
\item[$^{UnivAmsterdam}$] University of Amsterdam\\
\item[$^{CERN}$] CERN\\
\item[$^{KNU}$] Department of Physics, Kyungpook National University, Daegu, South Korea \\ 
\item[$^{UnivHouston}$] University of Houston \\
\end{itemize}

\textbf{Acknowledgements}~MvB acknowledge support from the Dutch NWO-I program 156, "Higgs as Probe and Portal". The work of A.J. is supported by the National Research Foundation of Korea, Grant No. NRF-2019R1A2C1009419. ~The work of J.~Mamuzic is supported in part by the Generalitat Valenciana (GV) through the  contract  APOSTD/2019/165, and by Spanish and European funds under the project PGC2018-094856-B-I00 (MCIU/AEI/FEDER, EU). 

==> authors-files/dilepton.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  J.~Bernigaud$^{IKP}$,
  J.~Bernigaud$^{TTP}$,
  A.~Bharucha$^{CPT}$,
  D.~Buttazzo$^{INFNPisa}$,
  J.~Dutta$^{RCAPP}$
  J.~Dutta$^{UH}$,
  D.~Marzocca$^{INFNTrieste}$,
  P.~Pani$^{DESYZ}$,
  G.~Polesello$^{INFNPavia}$,
  M.~Son$^{PhysKAIST}$,
  E.~Venturini$^{PhysTUM}$,
  N.~Vignaroli$^{FisPisa}$
\end{flushleft}

\begin{itemize}
\item[$^{IKP}$] Institute for Nuclear Physics (IKP), Karlsruhe Institute of Technology, Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\item[$^{CPT}$] CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{INFNPisa}$] INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{RCAPP}$]  Regional Centre for Accelerator-based Particle Physics, Harish-Chandra Research Institute, HBNI, Chhatnag Road, Jhunsi, Allahabad-211019, India
\item[$^{UH}$]  II. Institut f{\"u}r Theoretische Physik, Universit{\"a}t Hamburg, 
Luruper Chaussee 149, 22761 Hamburg, Germany
\item[$^{INFNTrieste}$] INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy
\item[$^{DESYZ}$] Deutsches Elektronen Synchrotron, DESY, 15738 Zeuthen, Germany
\item[$^{INFNPavia}$] INFN, Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy
\item[$^{PhysKAIST}$]  Department of Physics, Korea Advanced Institute of Science and Technology, 291 Daehak-ro, Yuseong-gu, Daejeon 34141, Republic of Korea,
\item[$^{PhysTUM}$] Physik- Department, TUM, 85748 Garching, Germany
\item[$^{FisPisa}$] Dipartimento di Fisica "E. Fermi", Università di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/higgseftobs.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  A.~Gilbert$^{NWU}$,
  J.~Langford$^{IC}$,
  N.~Wardle$^{IC}$
\end{flushleft}

\begin{itemize}
\item[$^{NWU}$] Northwestern University, Evanston, USA
\item[$^{IC}$] Imperial College, London, United Kingdom
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/lfu.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
    T.~BergerHrynova$^{LAPP}$,
    D.~Buttazzo$^{INFNPisa}$,
    J.~Dutta$^{RCAPP}$,
    J.~Dutta$^{UH}$,
    D.~Marzocca$^{INFNTrieste}$,
    M.~Son$^{PhysKAIST}$
\end{flushleft}

\begin{itemize}
\item[$^{INFNPisa}$] INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy,
\item[$^{LAPP}$] Univ.  Grenoble Alpes, Univ.  Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France
\item[$^{RCAPP}$] Regional Centre for Accelerator-based Particle Physics, Harish-Chandra Research Institute, HBNI, Chhatnag Road, Jhunsi, Allahabad-211019, India,
\item[$^{UH}$] II. Institut für Theoretische Physik, Universität Hamburg, Luruper Chaussee 149, 22761 Hamburg, Germany,
\item[$^{INFNTrieste}$]  INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy,
\item[$^{PhysKAIST}$]  Department of Physics, Korea Advanced Institute of Science and Technology, 291 Daehak-ro, Yuseong-gu, Daejeon 34141, Republic of Korea,
\end{itemize}

% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/likelihoodinfo.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  G.~Alguero$^{LPSC}$,
  J.~Y.~Araz$^{Concordia}$,
  B.~Fuks$^{LPTHE}$,
  B.~Fuks$^{IUF}$,
  S.~Kraml$^{LPSC}$,
  W.~Waltenberger$^{OeAW}$
\end{flushleft}

\begin{itemize}
\item[$^{LPSC}$] Laboratoire de Physique Subatomique et de Cosmologie, Universit\'e Grenoble-Alpes, CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{Concordia}$]  Concordia University 7141 Sherbrooke St. West, Montr\'eal, QC, Canada H4B 1R6
\item[$^{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE),UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{IUF}$]  Institut Universitaire de France, 103 boulevard Saint-Michel, 75005 Paris, France
\item[$^{OeAW}$] Institut f\"ur Hochenergiephysik, \"Osterreichische Akademie der Wissenschaften, Nikolsdorfer Gasse 18, 1050 Wien, Austria
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/recastcomp.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  J.~Y.~Araz$^{ConcordiaUniv}$,
  R.~Ruiz~de~Austri$^{IFIC}$,
  A.~Buckley$^{UnivGlasgow}$,
  N.~Desai$^{TIFR}$,
  B.~Fuks$^{LPTHE}$,
  B.~Fuks$^{IUF}$,
  T.~Gonzalo$^{Monash}$,
  P.~Gras$^{IRFU}$,
  A.~Kvellestad$^{ICL}$,
  A.~Kvellestad$^{UnivOslo}$,
  A.~Raklev$^{UnivOslo}$,
  S.~Sekmen$^{KNU}$
\end{flushleft}

\begin{itemize}
\item[$^{ConcordiaUniv}$] Department of Physics, Concordia University, Montr\'eal, Canada
\item[$^{IFIC}$] Instituto de F\'isica Corpuscular, CSIC-Universitat de Val\`encia, Spain
\item[$^{UnivGlasgow}$] School of Physics \& Astronomy, University of Glasgow, Scotland, UK
\item[$^{TIFR}$] Department of Theoretical Physics, Tata Institute of Fundamental Research, Mumbai, India
\item[$^{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies, Sorbonne Universit\'e et CNRS, Paris, France
\item[$^{IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{Monash}$] School of Physics and Astronomy, Monash University, Melbourne, VIC 3800, Australia
\item[$^{IRFU}$] CEA Institut de Recherche sur les lois Fondamentales de l'Univers, Universit\'e Paris-Saclay, Gif-sur-Yvette, France
\item[$^{ICL}$] Department of Physics, Imperial College London, UK
\item[$^{UnivOslo}$] Department of Physics, University of Oslo, Norway
\item[$^{KNU}$] Department of Physics, Kyungpook National University, Daegu, South Korea
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/singlelq.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  D.~Buttazzo$^{INFNPisa}$,
  D.~Marzocca$^{INFNTrieste}$,
  M.~Nardecchia$^{Sapienza}$,
  P.~Pani$^{DESYZ}$,
  G.~Polesello$^{INFNPavia}$,
\end{flushleft}

\begin{itemize}
\item[$^{INFNPisa}$] INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{INFNTrieste}$] INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy
\item[$^{Sapienza}$] Sapienza - Universita di Roma, Piazzale Aldo Moro 2, 00185, Roma, Italy
\item[$^{DESYZ}$] Deutsches Elektronen Synchrotron, DESY, 15738 Zeuthen, Germany
\item[$^{INFNPavia}$] INFN, Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> authors-files/tthz.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  S.~Banerjee$^{IPPP}$,
  R.~S.~Gupta$^{IPPP}$,
  S.~Jain$^{UM}$, 
  E.~Venturini$^{TUM}$
\end{flushleft}

\begin{itemize}
\item[$^{IPPP}$] Institute for Particle Physics Phenomenology, Department of Physics, Durham University, Durham DH1 3LE, United Kingdom
\item[$^{UM}$] School of Physics \& Astronomy, University of Minnesota, Minneapolis MN 55455, United States of America
\item[$^{TUM}$] Physik-Department, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }

 


==> contur/contur-update.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  A.~Buckley$^{Glasgow}$,
  J.~M.~Butterworth$^{UCL}$,
  L.~Corpe$^{UCL}$,
  G.~Watt$^{IPPP}$
  D.~Yallup$^{UCL}$
\end{flushleft}

\begin{itemize}
\item[$^{Glasgow}$] School of Physics and Astronomy, Glasgow University, Glasgow, UK
\item[$^{UCL}$] Department of Physics and Astronomy, UCL, London, WC1E 6BT, UK 
\item[$^{IPPP}$] Institute for Particle Physics Phenomenology, Durham University, Durham, UK 
\end{itemize}




==> contur/contur-update.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}


==> darkml/darkmachines.authors.tex <==
\begin{flushleft}
 M.~van Beekveld$^{HEF,\,Nikhef}$,
 S.~Caron$^{HEF,\,Nikhef}$,
 A.~De Simone$^{SISSA,\,INFN}$,
 A.~Farbin$^{UnivArlington}$,
 L.~Hendriks$^{HEF}$,
 A.~Jueid$^{UnivKonkuk}$,
 A.~Leinweber$^{UnivAdelaide}$,
 J.~Mamuzic$^{IFIC}$,
 E.~Mer\'enyi$^{UnivRice}$,
 A.~Morandini$^{SISSA,\,INFN}$,
 C.~Nellist$^{HEF,\,Nikhef}$,
 S.~Otten$^{HEF,\,UnivAmsterdam}$,
 M.~Pierini$^{CERN}$,
 R.~Ruiz de Austri$^{IFIC}$,
  J.~Schouwenberg$^{HEF,\,Nikhef}$,
 S.~Sekmen$^{KNU}$,
 R.~Vilalta$^{UnivHouston}$,
 M.~White$^{UnivAdelaide}$
\end{flushleft}

\begin{itemize}
\item[$^{HEF}$] HEF, Radboud University, Nijmegen, the Netherlands\\
\item[$^{Nikhef}$] Nikhef, Amsterdam, the Netherlands\\
\item[$^{SISSA}$] SISSA, Trieste, Italy\\
\item[$^{INFN}$] INFN, Trieste, Italy\\
\item[$^{UnivArlington}$] University of Texas Arlington\\
\item[$^{UnivKonkuk}$] School of Physics, Konkuk University, Seoul, Republic of Korea\\
\item[$^{UnivAdelaide}$] University of Adelaide \\
\item[$^{IFIC}$] Instituto de F\'isica Corpuscular, IFIC-UV/CSIC, Valencia, Spain \\
\item[$^{UnivRice}$] Rice University\\
\item[$^{UnivAmsterdam}$] University of Amsterdam\\
\item[$^{CERN}$] CERN\\
\item[$^{KNU}$] Department of Physics, Kyungpook National University, Daegu, South Korea \\ 
\item[$^{UnivHouston}$] University of Houston \\
\end{itemize}

\textbf{Acknowledgements}~MvB acknowledge support from the Dutch NWO-I program 156, "Higgs as Probe and Portal". The work of A.J. is supported by the National Research Foundation of Korea, Grant No. NRF-2019R1A2C1009419. ~The work of J.~Mamuzic is supported in part by the Generalitat Valenciana (GV) through the  contract  APOSTD/2019/165, and by Spanish and European funds under the project PGC2018-094856-B-I00 (MCIU/AEI/FEDER, EU). 

==> darkml/darkmachines.packages.tex <==
% packages
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{epsfig}
\usepackage{epsf}
\usepackage{epstopdf}
\usepackage[toc, page]{appendix}
\usepackage{bm}
\usepackage{dcolumn}
\usepackage[latin1]{inputenc}
\usepackage{rotating}
\usepackage{longtable}
\usepackage{enumerate}
\usepackage{tensor}
\usepackage{multirow}
\usepackage{url}
\usepackage[nonumberlist, nopostdot]{glossaries}
\usepackage{enumitem}


==> darkml/glossary.tex <==
\newglossaryentry{SM}
{
    name = Standard Model,
    description = {The model describing the dynamics and interactions of all known particles, in terms of quantum fields and symmetries. }
}
 
 
\newglossaryentry{QCD}
{
    name = Quantum Chromo-Dynamics (QCD),
    description = {The subset of the Standard Model describing the subnuclear strong force.}
}
 
\newglossaryentry{fourmom}
{
    name = 4-momentum,
    description = {The 4-dimensional vector describing energy $E$ and 3-dimensional momentum of a particle: $(E,\vec{p})=(E, p_x, p_y, p_z)$. }
}


\newglossaryentry{jet}
{
    name = Jet,
    description = {Quarks cannot exist on their own, and must combine to form hadrons, subatomic particles of two or more quarks which are bound together by the strong force. This process of forming hadrons is called hadronisation. A jet is a cone of hadrons that have been formed due to the hadronisation of quarks and gluons produced during the collisions in the LHC.}
}
 
\newglossaryentry{pt}
{
    name = Transverse momentum ($p_T$),
    description = {}
}

\newglossaryentry{xsec}
{
    name = Cross section,
    description = {}
}

\newglossaryentry{lumi}
{
    name = Luminosity,
    description = {}
}

\newglossaryentry{schannel}
{
    name = s-channel,
    description = {A scattering process where...}
}

\newglossaryentry{tchannel}
{
    name = t-channel,
    description = {}
}

\newglossaryentry{newphysics}
{
    name = New Physics,
    description = {The unknown physics lying beyond the Standard Model. }
}

\newglossaryentry{eta}
{
    name = Pseudo-rapidity ($\eta$),
    description = {In cylindrical coordinates,
    where $\hat z$ axis coincides with the protons beam line, 
    and the angular variables $\theta, \phi$ map the detector barrel, 
    the pseudo-rapidity is defined as $\eta \equiv-\ln\tan (\theta/2)$, 
    where $-\infty<\eta<+\infty$ for $\pi\geq \theta\geq 0$ (e.g. $\eta=0$ for
    $\theta=\pi/2$, and $\eta=+\infty$ for $\theta=0$).
    }
}

\newglossaryentry{phi}
{
    name = Azimuthal angle ($\phi$),
    description = {In cylindrical coordinates,
    where $\hat z$ axis coincides with the protons beam line, 
    and the angular variables $\theta, \phi$ map the detector barrel, 
    $\phi$ is the azimuthal angle.}
}

\newglossaryentry{gev}
{
    name = GeV,
    description = {Giga-ElectronVolts,
    corresponding to $10^9$ eV.}
}


==> dilepton/dilepton.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  J.~Bernigaud$^{IKP,TTP}$,
  A.~Bharucha$^{CPT}$,
  D.~Buttazzo$^{INFNPisa}$,
  J.~Dutta$^{RCAPP,UH}$,
  D.~Marzocca$^{INFNTrieste}$,
  P.~Pani$^{DESYZ}$,
  G.~Polesello$^{INFNPavia}$,
  E.~Venturini$^{PhysTUM}$,
  N.~Vignaroli$^{FisPisa}$
\end{flushleft}

\begin{itemize}
\item[$^{IKP}$] Institute for Nuclear Physics (IKP), Karlsruhe Institute of Technology, Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany,\\
\item[$^{TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany, \\
\item[$^{CPT}$] CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France, \\
\item[$^{INFNPisa}$] INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy, \\
\item[$^{RCAPP}$]  Regional Centre for Accelerator-based Particle Physics, Harish-Chandra Research Institute, HBNI, Chhatnag Road, Jhunsi, Allahabad-211019, India, \\
\item[$^{UH}$]  II. Institut f{\"u}r Theoretische Physik, Universit{\"a}t Hamburg, 
Luruper Chaussee 149, 22761 Hamburg, Germany, \\
\item[$^{INFNTrieste}$] INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy, \\
\item[$^{DESYZ}$] Deutsches Elektronen Synchrotron, DESY, 15738 Zeuthen, Germany, \\
\item[$^{INFNPavia}$] INFN, Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy, \\
\item[$^{PhysTUM}$] Physik- Department, TUM, 85748 Garching, Germany, \\
\item[$^{FisPisa}$] Dipartimento di Fisica "E. Fermi", Università di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy, 
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> filc/FILC.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  G.~B\'elanger$^{\rm LAPTh}$,
  A.~Bharucha$^{\rm CPT}$,
  N.~Desai$^{\rm TIFR}$, 
  B.~Fuks$^{\rm LPTHE, IUF}$,
  A.~Goudelis$^{\rm LPC}$,
  J.~Heisig$^{\rm CP3}$,
  A.~Lessa$^{\rm ABC}$,
  A.~Mjallal$^{\rm LAPTh}$,
  S.~Sekmen$^{\rm Kyungpook}$,
  D.~Sengupta$^{\rm UCSD}$,
  J. Zurita$^{\rm IKP, TTP}$  
\end{flushleft}

\begin{itemize}
\item[$^{\rm LAPTh}$] LAPTh, Univ.\ Grenoble Alpes, USMB, CNRS, 9 Chemin de Bellevue, F74940 Annecy, France
\item[$^{\rm CPT}$] CPT, UMR7332, CNRS and Aix-Marseille Universit\'{e} and Universit\'{e} de Toulon 13288 Marseille, France
\item[$^{\rm TIFR}$] Department of Theoretical Physics, Tata Institute of Fundamental Research, Homi Bhabha Road, Mumbai 400005, India
\item[$^{\rm LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{\rm IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{\rm LPC}$] Laboratoire de Physique de Clermont (UMR 6533), CNRS/IN2P3, Univ.\ Clermont Auvergne, 4 Av.\ Blaise Pascal, F-63178 Aubi\`ere Cedex, France
\item[$^{\rm CP3}$] Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{\rm ABC}$] Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil
\item[$^{\rm Kyungpook}$] Department of Physics, Kyungpook National University, Daegu, South Korea
\item[$^{\rm UCSD}$] Department of Physics and Astronomy, University of California, San Diego, 9500 Gilman Drive, La Jolla, U.S.A
\item[$^{\rm IKP}$] Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology, Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany
\item[$^{\rm TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology, Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> filc/FILC.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}
\usepackage[makeroom]{cancel}
\usepackage[compat=1.1.0]{tikz-feynman}

==> gwc/GWC.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  Jonathan~M.~Butterworth$^{1}$,
  Kenneth Lane$^{2}$, David Sperka$^{2}$
\end{flushleft}

\begin{itemize}
\item[$^{1}$] Department of Physics \& Astronomy, University College London, London, UK
\item[$^{2}$] Department of Physics, Boston University, Boston, MA 02215, USA
\end{itemize}


\title{Confronting the Higgs Bosons in Gildener-Weinberg Models with LHC
  Measurements}
\author{Jonathan~M.~Butterworth$^{1}$, Kenneth Lane$^{2}$}
\institute{
$^{1}$Department of Physics \& Astronomy, UCL, London, UK\\
$^{2}$Department of Physics, Boston University, Boston, MA 02215, USA
}



==> gwc/GWC.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}


==> higgseftobs/higgseftobs.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  A.~Gilbert$^{NWU}$,
  J.~Langford$^{IC}$,
  N.~Wardle$^{IC}$
\end{flushleft}

\begin{itemize}
\item[$^{NWU}$] Northwestern University, Evanston, USA
\item[$^{IC}$] Imperial College, London, United Kingdom
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> higgseftobs/higgseftobs.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}
% \usepackage{lineno}
% \linenumbers


==> lfu/lfu.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
    D.~Buttazzo$^{INFNPisa}$,
    J.~Dutta$^{RCAPP, UH}$,
    T.~Hryn'ova$^{LAPP}$,
    D.~Marzocca$^{INFNTrieste}$,
    M.~Son$^{PhysKAIST}$
\end{flushleft}

\begin{itemize}
\item[$^{INFNPisa}$] INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy,
\item[$^{LAPP}$] Univ.  Grenoble Alpes, Univ.  Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France
\item[$^{RCAPP}$] Regional Centre for Accelerator-based Particle Physics, Harish-Chandra Research Institute,
HBNI, Chhatnag Road, Jhunsi, Allahabad-211019, India,
\item[$^{UH}$] II. Institut für Theoretische Physik, Universität Hamburg, Luruper Chaussee 149, 22761 Hamburg, Germany,
\item[$^{INFNTrieste}$] 
INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy,
\item[$^{PhysKAIST}$] 
Department of Physics, Korea Advanced Institute of Science and Technology, 291 Daehak-ro,
Yuseong-gu, Daejeon 34141, Republic of Korea,
\end{itemize}

% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> lfu/lfu.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}


==> likelihood/likelihoodinfo.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  G.~Alguero$^{\rm LPSC}$,
  J.~Araz$^{\rm Concordia}$,
  B.~Fuks$^{\rm LPTHE,\ IUF}$,
  S.~Kraml$^{\rm LPSC}$,
  W.~Waltenberger$^{\rm OeAW}$
\end{flushleft}

\begin{itemize}
\item[$^{\rm LPSC}$] Laboratoire de Physique Subatomique et de Cosmologie, Universit\'e Grenoble-Alpes, CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{\rm Concordia}$]  Concordia University 7141 Sherbrooke St. West, Montr\'eal, QC, Canada H4B 1R6
\item[$^{\rm LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE),UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{\rm IUF}$]  Institut Universitaire de France, 103 boulevard Saint-Michel, 75005 Paris, France
\item[$^{\rm OeAW}$] Institut f\"ur Hochenergiephysik, \"Osterreichische Akademie der Wissenschaften, Nikolsdorfer Gasse 18, 1050 Wien, Austria
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> likelihood/likelihoodinfo.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}


==> llp-dm/LLP_DM.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\title{A common solution to $R_D$ anomalies and Dark Matter}
\begin{flushleft}
B.~Fuks$^{\rm LPTHE,\ IUF}$, 
J.~Heisig$^{\rm CP3}$, 
A.~Lessa$^{\rm UFABC}$, 
J.\,M.~No$^{\rm UAMCSIC}$,
S.~Sekmen$^{\rm KNU}$,
D.~Sengupta$^{\rm UCSD}$,
J.~Zurita$^{\rm IKP, TTP}$. 
\end{flushleft}

\begin{itemize}
\item[ $^{\rm LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^\text{IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{\rm CP3}$] Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{\rm UFABC}$] Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil,
\item[$^{\rm UAMCSIC}$] Departamento de Fisica Teorica and Instituto de Fisica Teorica, IFT-UAM/CSIC, Cantoblanco, 28049, Madrid, Spain,
\item[$^{\rm KNU}$] Kyungpook National University, Physics Dept., Daegu, South Korea.
\item[$^{\rm UCSD}$] Department of Physics and Astronomy, 9500 Gilman Drive, University of California, San Diego.
\item[$^{\rm IKP}$] Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany,
\item[$^{\rm TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology,  Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> llp-dm/LLP_DM.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}
\usepackage{lineno}


==> ml-1/PhenoAI.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  Sascha Caron$^{IMAPP,Nikhef}$, 
  Andrea Coccaro$^{INFN}$, 
  Sanmay Ganguly$^{WIS}$,
  Sabine Kraml$^{LPSC}$, 
  Andre Lessa$^{UFABC}$, 
  Sydney Otten$^{IMAPP,GRAPPA}$, 
  Humberto Reyes-Gonz\'{a}lez$^{LPSC}$, 
  Richard Ruiz$^{CP3}$, 
  Roberto Ruiz de Austri$^{IFC}$,
  Bob Stienen$^{IMAPP,Nikhef}$,
  Riccardo Torre$^{INFN}$
\end{flushleft}

\begin{itemize}
\item[$^{IMAPP}$]IMAPP, Radboud University, Nijmegen, the Netherlands
\item[$^{INFN}$]INFN, Sezione di Genova, Via Dodecaneso 33, I-16146 Genova, Italy
\item[$^{Nikhef}$]Nikhef, Amsterdam, the Netherlands
\item[$^{UFABC}$] Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil
\item[$^{CP3}$]Centre for Cosmology, Particle Physics and Phenomenology {\rm (CP3)}, Universit\'e Catholique de Louvain, Chemin du Cyclotron, Louvain la Neuve, B-1348, Belgium
\item[$^{LPSC}$]Laboratoire de Physique Subatomique et de Cosmologie, Universit\'{e} Grenoble-Alpes, \\ CNRS/IN2P3, 53 Avenue des Martyrs, F-38026 Grenoble, France
\item[$^{IFIC}$]Instituto de F\'isica Corpuscular, IFIC-UV/CSIC, Valencia, Spain.
\item[$^{GRAPPA}$]GRAPPA, University of Amsterdam, the Netherlands
\item[$^{WIS}$] Weizmann Institute of Science, Israel
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> ml-1/PhenoAI.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}
%\usepackage{appendix}
\usepackage{graphicx}
\usepackage{subfigure,slashed}
\usepackage{amsmath}
\usepackage{hyperref}
\usepackage{comment}
\usepackage{subfigure}

==> rdm/RDM.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\title{A common solution to $R_D$ anomalies and Dark Matter}
\begin{flushleft}
G.~B\'elanger$^{LAPTh}$, 
J.~Bernigaud$^{IKP,TTP}$, 
A.~Bharucha$^{Marseille}$, 
B.~Fuks$^{LPTHE,IUF}$, 
J.~Heisig$^{CP3}$, 
A.~Jueid$^{LAPTh}$, 
A.~Goudelis$^{LPC}$, 
A.~Lessa$^{UFABC}$, 
D.~Marzocca$^{TriesteINFN}$,
K.~A.~Mohan$^{MSU}$
M.~Nardecchia$^{Sapienza}$, 
G.~Polesello$^{PaviaINFN}$, 
P.~Pani$^{DesyZ}$, 
A.~Pukhov$^{MGU}$, 
D.~Sengupta$^{UCSD}$ 
J.~Zurita$^{IKP,TTP}$. 
\end{flushleft}

\begin{itemize}
\item[$^{LAPTh}$] LAPTh, Univ. Grenoble Alpes, USMB, CNRS, 9 Chemin de Bellevue, F-74940 Annecy, France,
\item[$^{IKP}$] Institute for Nuclear Physics (IKP), KIT Karlsruhe Institute of Technology,  Hermann-von-Helmholtz-Platz 1, D-76344 Eggenstein-Leopoldshafen, Germany,
\item[$^{TTP}$] Institute for Theoretical Particle Physics (TTP), Karlsruhe Institute of Technology,  Engesserstra{\ss}e 7, D-76128 Karlsruhe, Germany
\item[$^{Marseille}$] Aix Marseille Univ, Universit\'e de Toulon, CNRS, CPT, Marseille, F-13288 Marseille, France
\item[ $^{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^{\rm IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{CP3}$] Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, Chemin du Cyclotron 2, B-1348 Louvain-la-Neuve, Belgium
\item[$^{Konkuk}$] School of Physics, Konkuk University, 05029, Seoul, Republic of Korea
\item[$^{Clermont}$] Laboratoire de Physique de Clermont (UMR 6533), CNRS/IN2P3, Univ.\ Clermont Auvergne, 4 Av.\ Blaise Pascal, F-63178 Aubi\`ere Cedex, France,
\item[$^{ABC}$] Centro de Ci$\hat{e}$ncias Naturais e Humanas, Universidade Federal do ABC, Santo Andr\'e, 09210-580 SP, Brazil,
\item[$^{TriesteINFN}$] INFN Sezione di Trieste, via Bonomea 265, 34136 Trieste, Italy 
\item[$^{MSU}$]  Department of Physics and Astronomy, 567 Wilson Road,  East Lansing, Michigan-48824, USA
\item[$^{Sapienza}$] Sapienza - Universita di Roma, Piazzale Aldo Moro 2, 00185, Roma, Italy,
\item[$^{PaviaINFN}$] INFN, Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy,
\item[$^{DesyZ}$] Deutsches Elektronen Synchrotron, DESY, 15738 Zeuthen, Germany
\item[$^{MGU}$] Skobeltsyn Institute of Nuclear Physics, Moscow State University, Moscow 119992, Russia
\item[$^{UCSD}$] Department of Physics and Astronomy, 9500 Gilman Drive, University of California, San Diego.
%\item[$^{DeptLund}$] Department of Astronomy and Theoretical Physics, Lund University, Sweden
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> rdm/RDM.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}
\usepackage{lineno}


==> recastcomp/recastcomp.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  J.~Y.~Araz$^{\rm ConcordiaUniv}$,
  R.~Ruiz~de~Austri$^{\rm IFIC}$,
  A.~Buckley$^{\rm UnivGlasgow}$,
  N.~Desai$^{\rm TIFR}$,
  B.~Fuks$^{\rm LPTHE, IUF}$,
  T.~Gonzalo$^{\rm Monash}$,
  P.~Gras$^{\rm IRFU}$,
  A.~Kvellestad$^{\rm ICL, UnivOslo}$,
  A.~Raklev$^{\rm UnivOslo}$,
  S.~Sekmen$^{\rm KNU}$
\end{flushleft}

\begin{itemize}
\item[$^{\rm ConcordiaUniv}$] Department of Physics, Concordia University, Montr\'eal, Canada
\item[$^{\rm IFIC}$] Instituto de F\'isica Corpuscular, CSIC-Universitat de Val\`encia, Spain
\item[$^{\rm UnivGlasgow}$] School of Physics \& Astronomy, University of Glasgow, Scotland, UK
\item[$^{\rm TIFR}$] Department of Theoretical Physics, Tata Institute of Fundamental Research, Mumbai, India
\item[$^{\rm LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies, Sorbonne Universit\'e et CNRS, Paris, France
\item[$^{\rm IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^{\rm Monash}$] School of Physics and Astronomy, Monash University, Melbourne, VIC 3800, Australia
\item[$^{\rm IRFU}$] CEA Institut de Recherche sur les lois Fondamentales de l'Univers, Universit\'e Paris-Saclay, Gif-sur-Yvette, France
\item[$^{\rm ICL}$] Department of Physics, Imperial College London, UK
\item[$^{\rm UnivOslo}$] Department of Physics, University of Oslo, Norway
\item[$^{\rm KNU}$] Department of Physics, Kyungpook National University, Daegu, South Korea
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> recastcomp/recastcomp.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}


==> searchmeasurement/SearchMeasurementComplementarity.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  T.~Berger-Hryn'ova$^\text{LAPP}$,
  A.~Buckley$^\text{UGlasgow}$,
  J.~M.~Butterworth$^\text{UCL}$,
  L.~Corpe$^\text{UCL}$,
  D.~Yallup$^\text{UCL}$,
  M.~van Beekveld$^\text{UnivNijmegen}$,
  B.~Fuks$^\text{LPTHE,IUF}$,
  T.~Gonzalo$^\text{Monash}$,
  A.~Kvellestad$^\text{ICL,\,UnivOslo}$
\end{flushleft}

\begin{itemize}
\item[$^\text{LAPP}$] Univ.  Grenoble Alpes, Univ.  Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France
\item[$^\text{UGlasgow}$] School of Physics \& Astronomy, University of Glasgow, Scotland, UK
\item[$^\text{UCL}$] Department of Physics and Astronomy, University College London, UK
\item[$^\text{UnivNijmegen}$] Theoretical High Energy Physics, Radboud University Nijmegen, The Netherlands
\item[$^\text{LPTHE}$] Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), UMR 7589, Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France
\item[$^\text{IUF}$] Institut Universitaire de France, 103 boulevard Saint-Michel,  75005 Paris, France
\item[$^\text{Monash}$] School of Physics and Astronomy, Monash University, Melbourne, VIC 3800, Australia
\item[$^\text{ICL}$] Department of Physics, Imperial College London, UK
\item[$^\text{UnivOslo}$] Department of Physics, University of Oslo, Norway
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }


==> searchmeasurement/SearchMeasurementComplementarity.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}
\usepackage{ulem}
\usepackage{relsize}
\usepackage{listings}
\lstset{language=C++,
  basicstyle=\ttfamily\color{blue!50!black}\smaller,
  identifierstyle=\color{red!30!black},
  keywordstyle=\color{red!30!black},
  stringstyle=\color{green!30!black},
  breaklines=true,
  %postbreak=\mbox{\textcolor{red!30!black}{$\hookrightarrow$}\space}
}
%\lstMakeShortInline|


==> singlelq/singlelq.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  D.~Buttazzo$^{INFNPisa}$,
  D.~Marzocca$^{INFNTrieste}$,
  M.~Nardecchia$^{Sapienza}$,
  P.~Pani$^{DESYZ}$,
  G.~Polesello$^{INFNPavia}$,
\end{flushleft}

\begin{itemize}
\item[$^{INFNPisa}$] INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy, \\
\item[$^{INFNTrieste}$] INFN Sezione di Trieste, SISSA, Via Bonomea 265, 34136, Trieste, Italy, \\
\item[$^{Sapienza}$] Sapienza - Universita di Roma, Piazzale Aldo Moro 2, 00185, Roma, Italy,\\
\item[$^{DESYZ}$] Deutsches Elektronen Synchrotron, DESY, 15738 Zeuthen, Germany, \\
\item[$^{INFNPavia}$] INFN, Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy \\
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> vbf/VBF.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
  S.~Fichet$^{IIP}$,
  S.~Gascon-Shotkin$^{IPNL}$,
  A.~Lesauvage$^{IPNL}$, 
  G.~Moreau$^{IJCLab}$
\end{flushleft}

\begin{itemize}
\item[$^{IIP}$] International Institute of Physics, UFRN, Av. Odilon Gomes de Lima 1722 - Capim~Macio - 59078-400 - Natal-RN, Brazil
\item[$^{IPNL}$] Univ. Lyon, Universit\'e Claude Bernard Lyon 1, CNRS/IN2P3, UMR5822 IPNL F-69622 Villeurbanne, France
\item[$^{IJCLab}$] Laboratoire de Physique des 2 Infinis Ir\`ene Joliot-Curie d'Orsay (IJCLab), B\^at. 100, CNRS / PARIS-SACLAY, F-91898 ORSAY Cedex, France
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }

 

==> vbf/VBF.packages.tex <==
% add here the packages you used locally, 1 package per line
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{arydshln}
\usepackage{graphicx,epsfig}
\usepackage{color}  

==> vqlqvl/vq_lq_vl.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\title{Non-standard VLQ and LQ signatures from cascade decays}
\begin{flushleft}
J.~Butterworth$^1$,
G.~Cacciapaglia$^2$,
L.~Corpe$^1$,
T.~Flacke$^3$,
B.~Fuks$^{4,5}$,
L.~Panizzi$^6$, 
W.~Porod$^7$,
D.~Yallup$^1$
\end{flushleft}

\begin{itemize}
\item[$^1$] Department of Physics and Astronomy, University College London, London, WC1 6BT, UK.
\item[$^2$] Univ Lyon, Universit\'e Lyon 1, CNRS/IN2P3, IPNL, F-69622, Villeurbanne, France.
\item[$^3$] Center for Theoretical Physics of the Universe, Institute for Basic Science (IBS), Daejeon, 34126, Korea.
\item[$^4$] Laboratoire de Physique Th\'eorique et Hautes \'Energies (LPTHE), UMR 7589,
            Sorbonne Universit\'e et CNRS, 4 place Jussieu, 75252 Paris Cedex 05, France.
\item[$^5$] Institut Universitaire de France, 103 boulevard Saint-Michel, 75005 Paris, France.
\item[$^6$] Department of Physics and Astronomy, Uppsala University, Box 516, SE-751 20 Uppsala, Sweden.
\item[$^7$]  Uni.~W\"urzburg, Campus Hubland Nord, D-97074 W\"urzburg, Germany.
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }



==> wwtj/wwtj.authors.tex <==
% The content of this file will appear, locally, as a cover page of
% your contribution.  It won't be shown in the final report, but the
% information about your affiliation will be used by the editors to
% prepare the final report. Therefore, make sure your institute address
% is reported properly. We suggest to use the acronym of the institution or else identify it as DeptYourTown, etc..
%CERN,DESY,LAPTh,LAPP,IPPP,UCL,ICL,DeptTown,UnivTown
\begin{flushleft}
 A. Falkowski$^{IJCLab}$, 
 S. Ganguly$^{WIS}$, 
 P. Gras$^{\rm IRFU}$, 
 J. M. No$^{UAMCSIC}$
 K. Tobioka$^{FLD}$, 
 N. Vignaroli$^{FisPisa}$, 
 E. Venturini$^{PhysTUM}$, 
 T. You$^{CERN, Cam}$
\end{flushleft}

\begin{itemize}
\item[$^{IJCLab}$] Laboratoire de Physique des 2 Infinis Ir\`ene Joliot-Curie d'Orsay (IJCLab), B\^at. 100, CNRS / PARIS-SACLAY, F-91898 ORSAY Cedex, France
\item[$^{WIS}$] Weizmann Institute of Science, Israel
\item[$^{\rm IRFU}$] CEA  Institut  de  Recherche  sur  les  lois  Fondamentales  de  l'Univers,  Universit\'e  Paris-Saclay, Gif-sur-Yvette, France
\item[$^{UAMCSIC}$] Departamento de Fisica Teorica and Instituto de Fisica Teorica, IFT-UAM/CSIC, Cantoblanco, 28049, Madrid, Spain
\item[$^{FLD}$] Department of Physics, Florida State University, Tallahassee, FL 32306, USA
\item[$^{FisPisa}$] Dipartimento di Fisica "E. Fermi", Universit\'a di Pisa, and INFN Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy
\item[$^{PhysTUM}$] Physik-Department, Technische Universitat Munchen, 85748 Garching, Germany
\item[$^{CERN}$] CERN, Theoretical Physics Department, Geneva, Switzerland
\item[$^{Cam}$] DAMTP, University of Cambridge, Wilberforce Road, Cambridge, CB3 0WA, UK; Cavendish Laboratory, University of Cambridge, J.J. Thomson Avenue, Cambridge, CB3 0HE, UK
\end{itemize}


% \title{TITLE}
% \author{A.~Einstein$^{1}$, F.~Gauss$^{2}$}
% \institute{
% $^{1}$Institute for Particle Physics Phenomenology, Durham University, Durham, DH1 3LE, UK\\
% $^{2}$Department of Astronomy and Theoretical Physics, Lund University, Sweden
% }


